Advancements in Road Lane Mapping: Comparative Fine-Tuning Analysis of Deep Learning-based Semantic Segmentation Methods Using Aerial Imagery

This research addresses the need for high-definition (HD) maps for autonomous vehicles (AVs), focusing on road lane information derived from aerial imagery. While Earth observation data offers valuable resources for map creation, specialized models for road lane extraction are still underdeveloped in remote sensing. In this study, we perform an extensive comparison of twelve foundational deep learning-based semantic segmentation models for road lane marking extraction from high-definition remote sensing images, assessing their performance under transfer learning with partially labeled datasets. These models were fine-tuned on the partially labeled Waterloo Urban Scene dataset, and pre-trained on the SkyScapes dataset, simulating a likely scenario of real-life model deployment under partial labeling. We observed and assessed the fine-tuning performance and overall performance. Models showed significant performance improvements after fine-tuning, with mean IoU scores ranging from 33.56% to 76.11%, and recall ranging from 66.0% to 98.96%. Transformer-based models outperformed convolutional neural networks, emphasizing the importance of model pre-training and fine-tuning in enhancing HD map development for AV navigation.

==> 8parameter.tex <==
\begin{table*}[!h]
%\centering
\caption{FLOPS and Parameter Amount of 12 Models}
\label{tab:parameters}
\noindent
\begin{tabular}{lccc}
\toprule
Model       & Base & FLOPS & Parameters \\ \midrule
FCN         & ResNet101 & 276 G & 66.122 M \\
FastFCN     & ResNet50 & 94.604 G & 53.256 M \\
U-Net       & -        & 203 G & 28.987 M \\
DeepLabV3   & ResNet101 & 346 G & 84.718 M \\
DeepLabV3+  & ResNet101 & 254 G & 60.214 M \\
ANN         & ResNet101 & 263 G & 62.853 M \\
MobileNetV3 & Large & 8.771 G    & 3.284 M \\
PSPNet      & ResNet101 & 256 G & 65.599 M \\
SegNeXt     & Base & 34.498 G & 27.566 M \\
Twins       & Base & 70.232 G & 59.659 M \\
Swin        & Base & 305 G & 120 M \\
SegFormer   & Base & 74.596 G & 81.973 M \\
\bottomrule
\end{tabular}
\end{table*}

